Computing Threshold Circuits with Bimolecular Void Reactions in Step Chemical Reaction Networks

Step Chemical Reaction Networks (step CRNs) are an augmentation of the Chemical Reaction Network (CRN) model where additional species may be introduced to the system in a sequence of ``steps.'' We study step CRN systems using a weak subset of reaction rules, \emph{void} rules, in which molecular species can only be deleted. We demonstrate that step CRNs with only void rules of size (2,0) can simulate threshold formulas (TFs) under linear resources. These limited systems can also simulate threshold \emph{circuits} (TCs) by modifying the volume of the system to be exponential. We then prove a matching exponential lower bound on the required volume for simulating threshold circuits in a step CRN with (2,0)-size rules under a restricted \emph{gate-wise} simulation, thus showing our construction is optimal for simulating circuits in this way.

==> 2_0/2_0_circuits.tex <==
\vspace{-.4cm}

\section{Computation of Threshold Circuits with (2, 0) and (2, 1) Rules}\label{sec:2_0_formulas}
\vspace{-.2cm}

%Having established compatibility results of stepped CRNs with (3, 0) rules, we now examine stepped CRNs with a ruleset consisting of (2, 0) and (2, 1) catalyst rules. \textbf{[Should catalyst be defined here?]} We include the (2, 1) catalyst rules as there is no known way to strictly compute circuits with only (2, 0) rules.

%Section \ref{2_0_gates} shows how the computation of logic gates is still possible in stepped CRNs with (2, 0) and (2, 1) rules. We then demonstrate with Theorem \ref{(2,0)(2,1)_circuit} how the system can compute TC circuits with $O$($G$) species, $O$($D$) steps, and $O$($W$) volume.

Having established computation results with step CRNs using only true void rules, we now examine step CRNs whose rule-set also contains catalytic rules. %The combination of true and catalytic void rules in the system has some notable effects to the system's computation.
We discuss step CRNs consisting of (2, 0) and (2, 1) rules. Section \ref{2_0_gates} shows how the computation of logic gates is still possible in step CRNs with just (2, 0) rules. We then demonstrate with Theorem \ref{2_0_catalysts} how the system can compute TCs with $O(G)$ species, $O(D)$ steps, and $O(W)$ volume.

\vspace{-.3cm}
\subsection{Computing Logic Gates}\label{2_0_gates}
\vspace{-.2cm}

\para{Bit Representation.} The inputs of a binary gate are constructed the same as in Section \ref{3_0_gates}. Let $f_i^{in}$ be the set of all the indexes of the inputs fanning into a gate at index $i$. Let $f_i^{out}$ be the set of all the indexes of the inputs fanning out of a gate at index $i$.

The output of a gate is represented by the species $y_n^b$ or $y_{j \rightarrow i}^F$, where $j$ is the index of the input bit and $i$ is the index of the gate.

%Computing gates can be done with only (2, 0) rules. This method requires unique species to represent the inputs and outputs of each gate in a circuit. The species used to compute a particular gate should never be used to compute a different gate. Figure \ref{fig:(3,0)_figure} \textit{(b)} shows a pattern the gates can be indexed in. To compute an AND gate, we add a single copy of the species representing a true output ($y_{i}^T$) and a species representing the false output for each input fanning in ($\forall j \in f_i^{in}:$ $y_{j \rightarrow i}^F$). To compute an OR gate, we would add a species representing the true output for each input fanning in ($y_{j \rightarrow i}^T$) and a single $y_{i}^F$ species. To compute NOT gates, we would just add one copy of each output species ($y_i^b$). For all AND/OR/NOT gates, a rule should be made for every input fanning into a particular gate to delete the gate's output species with the opposite truth value to the input. If the output species has a unique $j \rightarrow i$ indexing, then only the input with the $i$th index can delete that output species.

\para{AND/OR/NOT Gate.}\label{2_0_basic_gates} Table \ref{tab:(2,0)_AND_OR_NOT} shows the general process to computing AND, OR, and NOT gates. %Computing gates is accomplished with only (2, 0) rules. This method requires unique species to represent the inputs and outputs of each gate in a circuit. The species used to compute a particular gate should never be used to compute a different gate. Figure \ref{fig:aoc1} shows a pattern the gates can be indexed in.
To compute an AND gate, we add a single copy of the species representing a true output ($y_{i}^T$) and a species representing the false output for each input fanning in ($\forall j \in f_i^{in}:$ $y_{j \rightarrow i}^F$). To compute an OR gate, we would add a species representing the true output for each input fanning in ($y_{j \rightarrow i}^T$) and a single $y_{i}^F$ species. To compute NOT gates, we would just add one copy of each output species ($y_i^b$). For all AND/OR/NOT gates, a rule should be made for every input fanning into a particular gate to delete the gate's output species with the opposite truth value to the input. If the output species has a unique $j \rightarrow i$ indexing, then only the input with the $i$th index can delete that output species.

%example AND gate
\para{OR Example.} Consider an OR gate at index $1$ with input bits 0 and 1. Here, $|f_i^{in}| = 2$ and the initial configuration consists of the species $x_1^F$ and a $x_2^T$. Following Table \ref{tab:(2,0)_AND_OR_NOT}, this gate can be computed in one step. 
%\vspace{-.1cm}
\begin{enumerate}
    \item One $y_{1 \rightarrow 1}^T$, one $y_{2 \rightarrow 1}^T$, and one $y_{1}^F$ species are added to the system. The species $x_2^T$ and $y_{1}^F$ delete each other. $x_1^F$ and $y_{1 \rightarrow 1}^T$ are also removed together. Only the species $y_{2 \rightarrow 1}^T$ remains, which represents the intended ``true'' output of the OR gate.
\end{enumerate}
\vspace{-.2cm}
%Table \ref{tab:(2,0)_AND_OR_NOT} shows how to compute a AND, OR, and NOT gate at index $i$. 

\begin{table}[t]
\vspace{-.2cm}
\renewcommand{\arraystretch}{.5}
\begin{center}
\begin{tabular}{ | c | c c | c | c | c c | c |}\hline

\textbf{Gate Type} & \multicolumn{2}{|c|}{\textbf{Step}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline

\textbf{AND} & \textit{Add} & \makecell{$y_{i}^T$ \\ $\forall j \in f_i^{in}:$ $y_{j \rightarrow i}^F$} & \makecell{$x_j^T + y_{j \rightarrow i}^F \rightarrow \emptyset$ \\ $x_j^F + y_i^T \rightarrow \emptyset$} & \makecell{An input species with a certain \\ truth value deletes the \\ complement output species.} \\ \hline

 \textbf{OR} & \textit{Add} & \makecell{$y_{i}^F$ \\ $\forall j \in f_i^{in}:$ $y_{j \rightarrow i}^T$} & \makecell{$x_j^T + y_i^F \rightarrow \emptyset$ \\ $x_j^F + y_{j \rightarrow i}^T \rightarrow \emptyset$} & \makecell{An input species with a certain \\ truth value deletes the \\ complement output species.} \\ \hline

 \textbf{NOT} & \textit{Add} & \makecell{$y_{i}^T$ \\ $y_{i}^F$} & \makecell{$x_j^T + y_i^T \rightarrow \emptyset$ \\ $x_j^F + y_i^F \rightarrow \emptyset$} & \makecell{The input and output species that \\ share the same truth value delete \\ each other.} \\ \hline

\end{tabular}

\caption{\textit{(2, 0) rules for AND, OR, and NOT gates.}}\label{tab:(2,0)_AND_OR_NOT}
\end{center}
\vspace{-.9cm}
\end{table}

%Let's consider the majority function when it has two unique input species, $T$ and $F$, where the counts of each species represent the amounts of true and false inputs, respectively. If $(|T| + |F|) \% 2 = 0$, then we should add an extra $F$ species before computing.

%The majority function can be computed with only (2, 0) rules if we add a rule where the T and F species delete each other: $T + F \rightarrow \emptyset$. With this rule, all of the minority species will be deleted and some amount of the majority species will remain.

%To implement a majority gate in a circuit with (2, 0) rules, we must first convert all input species ($x_n^b$) fanning into the gate at index $i$ into a new species that share the same index, which we will call $a_i^b$. If the amount of inputs fanning into a majority gate is even, then an extra false input should be fanned into that gate.

\vspace{-.2cm}
\para{Majority Gate.}\label{2_0_majority_gates} Table \ref{tab:(2,0)_MAJ} shows how to compute a majority gate at index $i$ (input index of some depth). To compute a majority gate, all input species are converted into a new species $a_{i}^b$ (step 1). The species retains the same index $i$ and truth value $b$ as the original input. If the number of species fanning into the majority gate is even, an extra false input species is added in. The species $b_{i}^b$ is then introduced, which computes the majority operation across all existing species. Any species that represent the minority inputs are deleted (step 2). The species remaining afterwards are then converted into the correct output species (step 3).


\begin{table}[t]
\vspace{-.2cm}
\renewcommand{\arraystretch}{.5}
\begin{center}
\begin{tabular}{| c | c  c | c | c |}\hline
    \multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline
    
    \textbf{1} & \textit{Add} & \makecell{$|f_i^{in}| \cdot a_i^T$ \\ $|f_i^{in}| \cdot a_i^F$} 
    
    & \makecell{\vspace{-10pt} \\ $\forall j \in f_i^{in}:$ \\ $x_j^T + a_i^F \rightarrow \emptyset$ \\ $x_j^F + a_i^T \rightarrow \emptyset$ \\ \vspace{-9pt}}
    
    & \makecell{$\forall j \in f_i^{in}$, convert $x_{j}^b$ input \\ species into $a_i^b$ species.} \\ \hline
    
    %%%
    \textbf{2} & \textit{Add} & \makecell{$\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^T$ \\ $\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^F$} 
    
    & \makecell{$a_i^T + b_i^F \rightarrow \emptyset$ \\ $a_i^F + b_i^T \rightarrow \emptyset$}
    
    & \makecell{Adding $\lfloor |f_i^{in}|/2 \rfloor$ amounts of $b_i^T$ and \\ $b_i^F$ species will delete all of the \\ minority species, leaving some amount \\ of the majority species remaining.} \\ \hline
    
    %%%
    \textbf{3} & \textit{Add} & \makecell{\vspace{-8pt} \\ $y_i^T$ \\ $y_i^F$ \\ \vspace{-10pt}} 
    
    & \makecell{$a_i^T + y_i^F \rightarrow \emptyset$ \\ $a_i^F + y_i^T \rightarrow \emptyset$}
    
    & \makecell{Convert $a_i^b$ into the proper output \\ species ($y_i^b$).} \\ \hline
    
\end{tabular}

\caption{\textit{(2, 0) rules for majority gates.}}\label{tab:(2,0)_MAJ}
\end{center}
\vspace{-1.3cm}
\end{table}


\vspace{-.3cm}
\subsection{Examples}\label{2_0_examples}
\vspace{-.2cm}

\input{2_0_example}


% \section{Powering Up (2, 0) Formulas to Circuits}\label{2_0_circuits}

% In this section, we continue to iterate on the (2, 0) stepped CRN model presented in Section \ref{2_0_formulas}. Altering certain characteristics of the system leads to improvements in the system's computation.

% Theorem \ref{(2,0)_circuit} shows how allowing for exponentially-sized volume in the system enables the computation of TC \textit{circuits} with $O$($G$) species, $O$($D$) steps, and $O$(${F_{out}}^D$) volume. We then seperately demonstrate how including catalyst rules into the system's ruleset allows for computation of TC circuits with only $O$($G$) species, $O$($D$) steps, and O($W$) volume in Theorem \ref{(2,0)(2,1)_circuit}.

% \subsection{Exponential Volume}\label{2_0_exp_vol}

% \begin{theorem}\label{(2,0)_circuit}
% Boolean circuits (TC) can be computed with multiple input relaxed by a step CRN with only (2, 0) rules, O(G) species, O(D) steps, and O(${F_{out}}^D$) volume.
% \end{theorem}
% \begin{proof}
% %\textit 
% %To handle circuits, a CRN must handle fan out. The simplest way to handle fan out is to copy it and everything underneath it into 2 sections. One is to simulate one output of the gate, and another is  to simulate the other output of the gate. All this truly does is drag the fan out back to the beginning, but if given enough copies of the inputs, this can be done. It comes at the cost of 2 to the depth power species because each new set of identical gates must have different species. It is more efficient to not divide the circuit, but instead run more inputs through each gate. A 2,0 step crn cannot double something, but it can, given twice the inpts, create twice as much of it.If we put 4 inputs into an and gate by using there rules (need picture of professor bins 2,0 solution below this) instead of two, we end up with 2 outputs. by adding a step to separate the two, we can reset the next level to simply have normal inputs. This simulates circuits in volume = 2 to depth instead of species = 2 to depth because we do not need new species for each fanout, only more of the inputs. The specific metrics are 4Depth steps, 6Gate species, and 2 to the depth power volume. This method is unnatural because it requires more then 1 copy of each input bit.

% There is no known way to duplicate a single species with only (2, 0) rules and strict computing. So, to create enough copies of the output of a gate that fans out, we must increase the count of the inputs to match the count of the gate or sum of gates it is being inputted into. For instance, if a gate needs $k$ copies of its output species to fan out, each of the gates that are inputs for that gate also needs $k$ copies of their output species, and each of the gates that are inputs for those gates needs $k$ copies, and so on. The counts of the species that are added in each step ($x_i^b$ and $y_i^b$) also need to be multiplied by the number of output species a given gate needs.

% \textbf{Big-Oh Complexity Analysis:} The species and steps Big-Oh complexity (O(G) and O(D), respectively) remain unchanged from the method used to compute formulas because no new species or steps are being introduced.

% The volume of the system could grow exponentially based on the depth and the size of the max fan out. For instance, if the primary inputs were inputted into a gate that had a fan out of $k$, and that gate fanned out into other gates that had a fan out of $k$, and this pattern continued for most of the circuit, then the primary input species' count would need to be multiplied by $k$ for the amount of depth levels this pattern continued. Therefore, where $F_{out}$ is the max fan out of a circuit, then a circuit simulation could require a O(${F_{out}}^D$) volume.
% \end{proof}


% %\begin{theorem}
% %Parity functions can be naturally simulated by a 2-step CRN with only (2, 0) rules \textbf{(SPECIES METRICS)}.
% %\end{theorem}
% %\begin{proof}
% %\textit I believe this one doesn't matter anymore because of the 1 step 2,0 solution.
% %\end{proof}

\vspace{-.2cm}
\subsection{Computing Circuits with Catalyst Rules}\label{2_0_catalysts}
\vspace{-.1cm}

\begin{theorem} \label{(2,0)(2,1)_circuit}
Threshold circuits (TC) can be strictly computed by $(2,1)$ catalyst rules and $(2,0)$ void rules using O(G) species, O(D) steps, and O(W) volume.
\end{theorem}


\begin{proof}
%The use of (2, 1) catalyst rules enables the CRN to preserve an input for reuse multiple times at the same gate. This allows for fanout into multiple outputs without needing to increase the quantity of input species, enabling strict simulation. For a gate with output $z$, the number of $z_0$ and $z_1$ species as well as any other needed species for the step process can be added in quantities equal to the outdegree of the gate, and the gate will produce the correct output in that quantity.
%Consider an AND gate that has two input bits $x$ and $y$, and output bits $z$. 

%We have the rules $x_0+z_1\rightarrow x_0$, $y_0+z_1\rightarrow y_0$ to deal with the cases that one of $x$ and $y$ is $0$.

%For the case that both input bits are $1$, we have the following rules over three steps:
%\begin{enumerate}
%  \item  $c$, $d$ are added: $x_1+c\rightarrow x_1$ and $y_1+d\rightarrow y_1$
%  \item $e$ is added: $c+e\rightarrow \emptyset$ and $d+e\rightarrow \emptyset$
%  \item $z_0, z_1$ are added: $e+z_0\rightarrow \emptyset$
%\end{enumerate}

%For the case of a NOT gate with input $x$ and output $z$. We have the rules $x_0+z_0\rightarrow x_0$, and $x_1+z_1\rightarrow x_1$.

%An OR gate with input bits $x$ and $y$ and output bits $z$ works similarly to an AND gate.

%The rules $x_1+z_0\rightarrow x_1$ and $y_1+z_0\rightarrow y_1$ handle if either input is $1$.

%For the case that both inputs are $0$, we have the following rules over three steps:
%\begin{enumerate}
%  \item $f,g$ are added: $x_0+f\rightarrow x_0$ and $y_0+g\rightarrow y_0$
%  \item $h$ is added: $f+h\rightarrow \emptyset$ and $g+h\rightarrow \emptyset$
%  \item $z_0, z_1$ are added: $h+z_1\rightarrow \emptyset$
%\end{enumerate}

%This approach can also handle fan-in by increasing the number of rules and helper species to match the fan-in of a gate. In the AND gate example, if either of the two inputs $x$ or $y$ is 0, then $z_1$ is deleted. If the gate were to have a third input $w$, then a rule can be added where $w_0+z_1\rightarrow \emptyset$. Additionally, helper species $c$ and $d$ are consumed in catalyst reactions when $x$ or $y$ are 1. Another species $b$ can be added in step 1 to react with $w$ if it is 1 where $w_1+b\rightarrow\emptyset$. If $w$ is 0, species $b$ will not be deleted and in step two, a rule can be added where $b+e\rightarrow\emptyset$. Thus species $e$ will still only be present to delete $z_0$ if all three inputs are 1. This approach can be expanded as needed to handle larger fan-in, and a similar approach can be used for OR gates.

%Because the species for each gate are unique, one depth level can be handled at a time. This allows for D steps and G species, where a unique species is used for each initial input to the circuit and for each output of a gate. The number of species added during any step will depend on the width of the circuit at that depth level, and their quantities will correspond to the fanout of the gates at that level. However, due to catalyst rules the inputs of gates will not be deleted. Only helper species and incorrect versions of output species are deleted by void rules. Thus the volume of this simulation would be O(G).


With only (2, 0) rules, there is no known way to perform fan-outs without introducing, at most, an exponential amount of species at certain steps. This makes it impossible to strictly compute circuits with only (2, 0) rules and results in a large volume. The use of (2, 1) catalyst rules enables the step CRN to compute with arbitrary fan-out without an increase in species count, as well as deleting all species that are no longer needed. This allows for strict computation and decreases the volume of the step CRN to a polynomial size.

The initial configuration of this step CRN should consist of a $y_n^b$ species with the appropriate indexing and truth values for each primary input. Section \ref{2_0_gates} explains how to compute TC gates. To run the circuit, we must convert the output species into input species. In addition, this step CRN uses ``deleting'' species $d_x$ and $d_y$ that remove species that are no longer needed. Table \ref{tab:cat_fan_out} shows the steps and rules needed to perform arbitrary fan-out for a gate at index $i$. All outputs at the same depth level can be fanned out at the same time.

\begin{table}[t]
\vspace{-.2cm}
\renewcommand{\arraystretch}{.5}
    \begin{center}
    \begin{tabular}{| c | c  c | c | c |}\hline
    
    \multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline
    
    \textbf{1} & \textit{Add} & \makecell{$d_x$} 
    
    & \makecell{\vspace{-8pt} \\ $\forall n \in \{1,\cdots,G\}:$ \\ $\forall b \in \{T,F\}$ \\ $d_x + x_n^b \rightarrow d_x$ \\ $d_x + a_n^b \rightarrow d_x$ \\ $d_x + b_n^b \rightarrow d_x$ \\ \vspace{-8pt}}
    
    & \makecell{Delete all input species ($x_n^b$) and helper \\ species that are no longer needed.} \\ \hline
    
    %%
    \textbf{2} & \textit{Add} & \makecell{$d_x$} 
    
    & \makecell{\vspace{-8pt} \\ $d_x + d_x \rightarrow \emptyset$ \\ \vspace{-8pt}}
    
    & \makecell{Remove deleting species $d_x$.} \\ \hline
    
    %%
    \textbf{3} & \textit{Add} & \makecell{$|f_i^{out}| \cdot x_i^T$ \\ $|f_i^{out}| \cdot x_i^F$} 
    
    & \makecell{\vspace{-8pt} \\ $y_i^T + x_i^F \rightarrow y_i^T$ \\ $y_i^F + x_i^T \rightarrow y_i^F$ \\ $\forall j \in f_i^{in}:$ \\ $y_{j \rightarrow i}^T + x_i^F \rightarrow y_{j \rightarrow i}^T$ \\ $y_{j \rightarrow i}^F + x_i^T \rightarrow y_{j \rightarrow i}^F$ \\ \vspace{-8pt}}
    
    & \makecell{Add species representing true and false \\ inputs and delete the species that are the \\ complement of the output. A single output \\ species can assign the truth value for as \\ many input species as needed.} \\ \hline
    
    %%
    \textbf{4} & \textit{Add} & \makecell{$d_y$} 
    
    & \makecell{\vspace{-8pt} \\ $\forall n \in \{1,\cdots,G\}:$ \\ $d_y + y_n^T \rightarrow d_y$ \\ $d_y + y_n^F \rightarrow d_y$ \\ $\forall j \in f_i^{in}:$ \\ $d_y + y_{j \rightarrow i}^T \rightarrow d_y$ \\ $d_y + y_{j \rightarrow i}^F \rightarrow d_y$ \\ \vspace{-8pt}}
    
    & \makecell{Delete all output species ($y_n^b$) that no \\ longer needed.} \\ \hline
    
    %%
    \textbf{5} & \textit{Add} & \makecell{$d_y$} 
    
    & \makecell{\vspace{-8pt} \\ $d_y + d_y \rightarrow \emptyset$ \\ \vspace{-8pt}}
    
    & \makecell{Remove deleting species $d_y$.} \\ \hline
    
    \end{tabular}
    
    \caption{\textit{(2, 0) and (2, 1) rules and steps for a gate with arbitrary fan out.}}\label{tab:cat_fan_out}
\end{center}
\vspace{-1.3cm}
\end{table}

\textbf{Complexity:} Having a constant amount of unique species represent each gate in a circuit and a constant number of helper species results in $O(G)$ species.
All gates at a given depth level are computed at the same time in a constant number of steps. Thus, the circuit simulation requires $O(D)$ steps.
This step CRN only needs to introduce a constant number of species to compute each gate, and it deletes all species no longer needed after computing all gates at a given depth level. Thus, the step CRN  requires $O(W)$ volume.
\end{proof}




==> 2_0/2_0_circuits_exponential.tex <==
\section{Powering Up (2, 0) Formulas to Circuits}\label{2_0_circuits}

In this section, we continue to iterate on the (2, 0) stepped CRN model presented in Section \ref{2_0_formulas}. Altering certain characteristics of the system leads to improvements in the system's computation.

Theorem \ref{(2,0)_circuit} shows how allowing for exponentially-sized volume in the system enables the computation of TC \textit{circuits} with $O$($G$) species, $O$($D$) steps, and $O$(${F_{out}}^D$) volume. We then seperately demonstrate how including catalyst rules into the system's ruleset allows for computation of TC circuits with only $O$($G$) species, $O$($D$) steps, and O($W$) volume in Theorem \ref{(2,0)(2,1)_circuit}.

\subsection{Exponential Volume}\label{2_0_exp_vol}

\begin{theorem}\label{(2,0)_circuit}
Boolean circuits (TC) can be computed with multiple input relaxed by a step CRN with only (2, 0) rules, O(G) species, O(D) steps, and O(${F_{out}}^D$) volume.
\end{theorem}
\begin{proof}
%\textit 
%To handle circuits, a CRN must handle fan out. The simplest way to handle fan out is to copy it and everything underneath it into 2 sections. One is to simulate one output of the gate, and another is  to simulate the other output of the gate. All this truly does is drag the fan out back to the beginning, but if given enough copies of the inputs, this can be done. It comes at the cost of 2 to the depth power species because each new set of identical gates must have different species. It is more efficient to not divide the circuit, but instead run more inputs through each gate. A 2,0 step crn cannot double something, but it can, given twice the inpts, create twice as much of it.If we put 4 inputs into an and gate by using there rules (need picture of professor bins 2,0 solution below this) instead of two, we end up with 2 outputs. by adding a step to separate the two, we can reset the next level to simply have normal inputs. This simulates circuits in volume = 2 to depth instead of species = 2 to depth because we do not need new species for each fanout, only more of the inputs. The specific metrics are 4Depth steps, 6Gate species, and 2 to the depth power volume. This method is unnatural because it requires more then 1 copy of each input bit.

There is no known way to duplicate a single species with only (2, 0) rules and strict computing. So, to create enough copies of the output of a gate that fans out, we must increase the count of the inputs to match the count of the gate or sum of gates it is being inputted into. For instance, if a gate needs $k$ copies of its output species to fan out, each of the gates that are inputs for that gate also needs $k$ copies of their output species, and each of the gates that are inputs for those gates needs $k$ copies, and so on. The counts of the species that are added in each step ($x_i^b$ and $y_i^b$) also need to be multiplied by the number of output species a given gate needs.

\textbf{Big-Oh Complexity Analysis:} The species and steps Big-Oh complexity (O(G) and O(D), respectively) remain unchanged from the method used to compute formulas because no new species or steps are being introduced.

The volume of the system could grow exponentially based on the depth and the size of the max fan out. For instance, if the primary inputs were inputted into a gate that had a fan out of $k$, and that gate fanned out into other gates that had a fan out of $k$, and this pattern continued for most of the circuit, then the primary input species' count would need to be multiplied by $k$ for the amount of depth levels this pattern continued. Therefore, where $F_{out}$ is the max fan out of a circuit, then a circuit simulation could require a O(${F_{out}}^D$) volume.
\end{proof}


%\begin{theorem}
%Parity functions can be naturally simulated by a 2-step CRN with only (2, 0) rules \textbf{(SPECIES METRICS)}.
%\end{theorem}
%\begin{proof}
%\textit I believe this one doesn't matter anymore because of the 1 step 2,0 solution.
%\end{proof}

\subsection{Computing Circuits with Catalyst Rules}\label{2_0_catalysts}

%Rachel is looking into Dr. Fu's work on this
\begin{theorem} \label{(2,0)(2,1)_circuit}
Boolean circuits (TC) can be strictly computed by $(2,1)$ catalyst rules and $(2,0)$ void rules using O(G) species, O(D) steps, and O(W) volume.
\end{theorem}

\begin{proof}
%The use of (2, 1) catalyst rules enables the CRN to preserve an input for reuse multiple times at the same gate. This allows for fanout into multiple outputs without needing to increase the quantity of input species, enabling strict simulation. For a gate with output $z$, the number of $z_0$ and $z_1$ species as well as any other needed species for the step process can be added in quantities equal to the outdegree of the gate, and the gate will produce the correct output in that quantity.
%Consider an AND gate that has two input bits $x$ and $y$, and output bits $z$. 

%We have the rules $x_0+z_1\rightarrow x_0$, $y_0+z_1\rightarrow y_0$ to deal with the cases that one of $x$ and $y$ is $0$.

%For the case that both input bits are $1$, we have the following rules over three steps:
%\begin{enumerate}
%  \item  $c$, $d$ are added: $x_1+c\rightarrow x_1$ and $y_1+d\rightarrow y_1$
%  \item $e$ is added: $c+e\rightarrow \emptyset$ and $d+e\rightarrow \emptyset$
%  \item $z_0, z_1$ are added: $e+z_0\rightarrow \emptyset$
%\end{enumerate}

%For the case of a NOT gate with input $x$ and output $z$. We have the rules $x_0+z_0\rightarrow x_0$, and $x_1+z_1\rightarrow x_1$.

%An OR gate with input bits $x$ and $y$ and output bits $z$ works similarly to an AND gate.

%The rules $x_1+z_0\rightarrow x_1$ and $y_1+z_0\rightarrow y_1$ handle if either input is $1$.

%For the case that both inputs are $0$, we have the following rules over three steps:
%\begin{enumerate}
%  \item $f,g$ are added: $x_0+f\rightarrow x_0$ and $y_0+g\rightarrow y_0$
%  \item $h$ is added: $f+h\rightarrow \emptyset$ and $g+h\rightarrow \emptyset$
%  \item $z_0, z_1$ are added: $h+z_1\rightarrow \emptyset$
%\end{enumerate}

%This approach can also handle fan-in by increasing the number of rules and helper species to match the fan-in of a gate. In the AND gate example, if either of the two inputs $x$ or $y$ is 0, then $z_1$ is deleted. If the gate were to have a third input $w$, then a rule can be added where $w_0+z_1\rightarrow \emptyset$. Additionally, helper species $c$ and $d$ are consumed in catalyst reactions when $x$ or $y$ are 1. Another species $b$ can be added in step 1 to react with $w$ if it is 1 where $w_1+b\rightarrow\emptyset$. If $w$ is 0, species $b$ will not be deleted and in step two, a rule can be added where $b+e\rightarrow\emptyset$. Thus species $e$ will still only be present to delete $z_0$ if all three inputs are 1. This approach can be expanded as needed to handle larger fan-in, and a similar approach can be used for OR gates.

%Because the species for each gate are unique, one depth level can be handled at a time. This allows for D steps and G species, where a unique species is used for each initial input to the circuit and for each output of a gate. The number of species added during any step will depend on the width of the circuit at that depth level, and their quantities will correspond to the fanout of the gates at that level. However, due to catalyst rules the inputs of gates will not be deleted. Only helper species and incorrect versions of output species are deleted by void rules. Thus the volume of this simulation would be O(G).



The issue simulating a circuit with only (2, 0) rules is that there is no known way to perform fan-outs without introducing, at most, an exponential amount of species at certain steps. There is also no known way to compute a circuit in such a way that all of the species that are no longer needed will always be deleted. This could result in the increasing volume after each step. The use of (2, 1) catalyst rules enables the step CRN to compute with arbitrary fan-out without an increase in species count, as well as delete all species that are no longer needed. This decreases the volume of the step CRN to a significantly more manageable size.

To compute gates, this step CRN adopts all of the methods used by a step CRN with only (2, 0) rules (see Section \ref{2_0_gates}). In addition, this step CRN uses deleter species $d_x$ and $d_y$ that remove species that are no longer needed. To run the circuit, we must convert the output species into input species using a slightly different method from the one shown in Theorem \ref{(2,0)_formula}. The steps and rules shown below demonstrate an arbitrary fan-out for a gate at index $i$. All outputs at the same depth level can be fanned out at the same time.

\begin{table}[t]
    \begin{center}
    \begin{tabular}{| c | c  c | c | c |}\hline
    
    \multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline
    
    \textbf{1} & \textit{Add} & \makecell{$d_x$} 
    
    & \makecell{\vspace{-8pt} \\ $\forall n \in \{1,\cdots,G\}:$ \\ $\forall b \in \{T,F\}$ \\ $d_x + x_n^b \rightarrow d_x$ \\ $d_x + a_n^b \rightarrow d_x$ \\ $d_x + b_n^b \rightarrow d_x$ \\ \vspace{-8pt}}
    
    & \makecell{Delete all input species ($x_n^b$) and helper \\ species that are no longer needed.} \\ \hline
    
    %%
    \textbf{2} & \textit{Add} & \makecell{$d_x$} 
    
    & \makecell{\vspace{-8pt} \\ $d_x + d_x \rightarrow \emptyset$ \\ \vspace{-8pt}}
    
    & \makecell{Remove deleter species $d_x$.} \\ \hline
    
    %%
    \textbf{3} & \textit{Add} & \makecell{$\forall k \in f_i^{out}:$ \\ $x_k^T$ \\ $x_k^F$} 
    
    & \makecell{\vspace{-8pt} \\ $\forall k \in f_i^{out}:$ \\ $y_i^T + x_k^F \rightarrow y_i^T$ \\ \underline{$y_i^F + x_k^T \rightarrow y_i^F$} \\ $\forall j \in f_i^{in}:$ \\ $y_{j \rightarrow i}^T + x_k^F \rightarrow y_{j \rightarrow i}^T$ \\ $y_{j \rightarrow i}^F + x_k^T \rightarrow y_{j \rightarrow i}^F$ \\ \vspace{-8pt}}
    
    & \makecell{Add species representing true and false \\ inputs and delete the species that are the \\ complement of the output. A single output \\ species can assign the truth value for as \\ many different input species as needed.} \\ \hline
    
    %%
    \textbf{4} & \textit{Add} & \makecell{$d_y$} 
    
    & \makecell{\vspace{-8pt} \\ $\forall n \in \{1,\cdots,G\}:$ \\ $d_y + y_n^T \rightarrow d_y$ \\ \underline{$d_y + y_n^F \rightarrow d_y$} \\ $\forall j \in f_i^{in}:$ \\ $d_y + y_{j \rightarrow i}^T \rightarrow d_y$ \\ $d_y + y_{j \rightarrow i}^F \rightarrow d_y$ \\ \vspace{-8pt}}
    
    & \makecell{Delete all output species ($y_n^b$) that no \\ longer needed.} \\ \hline
    
    %%
    \textbf{5} & \textit{Add} & \makecell{$d_y$} 
    
    & \makecell{\vspace{-8pt} \\ $d_y + d_y \rightarrow \emptyset$ \\ \vspace{-8pt}}
    
    & \makecell{Remove deleter species $d_y$.} \\ \hline
    
    \end{tabular}
    
    \caption{\textit{(2, 0) and (2, 1) rules for a circuit.}}\label{tab:cat_fan_out}
\end{center}
\end{table}

\textbf{Big-Oh Complexity Analysis:} This step CRN only introduces the species $d_x$ and $d_y$. All other species are adopted from the step CRN with only (2, 0) rules. Therefore, this step CRN would require O($G$) species.

Compared to the step CRN with only (2, 0) rules, this step CRN introduces a constant amount of new steps per depth level. Therefore, this circuit simulation would require O($D$) steps.

This step CRN only needs to introduce a constant amount of species to compute each gate, and it deletes all species no longer needed after computing all gates at a given depth level. Therefore, this step CRN would require O($W$) volume.
\end{proof}


\section{Impossiblity for Conventional CRN}

In this section, we show that it is impossible to simulate the parity function using a conventional CRN, which is a step CRN with one step. The parity function parity$_n(x_1,x_2,\cdots, x_n):\{0,1\}^n\rightarrow \{0,1\}$ is $1$ if $x_1+x_2+\cdots+x_n$ is odd, and $0$ otherwise. 

A {\it separated strict CRN} is a   strict CRN $C_S=(S, X, Y)$ such that the there is no overlap between $X$ and $Y$. In other words, the output species are not from the input species. In particular, a separated strict CRN $(S, X, Y)$ computes a boolean function where $f(x_1,\cdots, x_n)=y_1:\{0,1\}^n\rightarrow \{0,1\}$ has $Y=((y_1^0, y_1^1))$. We denote $C(z)$ the number of copies of $z^0$ and $z^1$ added to a separated strict CRN $(S, X, Y)$. Define $L(C_S)$ to be the largest $i$ such that there is a rule in $C_S$ of size $(i,j)$ for some integers $i, j$.


\begin{theorem}
For a separated strict CRN $C_s=(S,X, Y)$ with $Y=((y_1^0, y_1^1))$ and catalyst rules, if $L(C_S) C(y_1)<n$, then $C_s$ cannot  compute a parity$_n(.)$ in one step.
\end{theorem}

\begin{proof}
Assume that a separated strict CRN $C_s=(S,X, Y)$ computes parity$_n(.)$ that outputs $y_1^0$ or $y_1^1$ for $0$ and $1$ respectively. Assume $n$ is odd. We must have rules $R_1,\cdots, R_t$ that remove $y_1^0$ when computing parity$_n(1,1,\cdots, 1)$. Clearly, $t\le C(y_1)$ since we have at most $C(y_1)$ copies of $y_1^0$. Since $L(C_S) C(y_1)<n$, there is a $(x_i^0, x_i^1)$ in $X$ that is not accessed by the $t$ rules $R_1,\cdots, R_t$.  Flipping $x_i^1$ to $x_i^0$ in the input, the same $t$ rules can still be applied, and all copies for $y_1^0$ are removed. This leaves $y_1^1$ as the output. Now the number of $1$ in the input bits is even. This gives a contradiction.
\end{proof}

==> 2_0/2_0_formulas.tex <==
\section{Computation of Threshold Formulas with (2, 0) Rules}\label{2_0_formulas}

We now examine stepped CRNs with a ruleset consisting of (2, 0) rules instead. Decreasing the reactant count of the void rules has some notable changes to the system's computation.

Section \ref{2_0_gates} shows how the computation of logic gates is still possible in stepped CRNs with (2, 0) rules. We then demonstrate with Theorem \ref{(2,0)_formula} how the system can compute TC \textit{formulas} (but not circuits) with $O$($G$) species, $O$($D$) steps, and $O$($G$) volume.

\subsection{Computing Logic Gates}\label{2_0_gates}
%(2, 0) CRN's are not capable of hard coding a two-input gate. We can not consider both inputs and destroy an output based on them. This limits us to reactions that can only include one of the inputs. Our solution is achieved by manipulating the outputs. given an and gate, any 1 input deletes a 0 output, and any 0 input deletes a 1 output. The number of 0 outputs is equal to the number of inputs because all inputs must be 1 for an and gate to not return 0.

The inputs of a binary gate in a step CRN systems are constructed the same as in Section \ref{3_0_gates}. Let $f_i^{in}$ be the set of all the indexes of the inputs fanning into a gate at index $i$. Let $f_i^{out}$ be the set of all the indexes of the inputs fanning out of a gate at index $i$.

The outputs of gates in a step CRN system with (2, 0) rules are represented by either the species $y_n^b$ or $y_{i \rightarrow j}^F$.

\subsubsection{Basic Gates}\label{2_0_basic_gates}

Computing gates with (2, 0) rules requires an unique species for representing the inputs and outputs of each gate in a circuit. The species that are used to compute a particular gate, should never be used to compute a different gate. Figure \ref{fig:(3,0)_figure} \textit{(b)} shows a pattern the gates can be indexed in. To compute an AND gate, we add a single copy of the species representing a true output ($y_{j}^T$) and a species representing the false output for each input fanning in ($y_{i \rightarrow j}^F$, where $i$ is the index of the input). To compute an OR gate, we would add a species representing the true output for each input fanning in ($y_{i \rightarrow j}^T$) species and a single $y_{j}^F$ species. To compute NOT gates, we  just need to add one copy of each output species. For all AND/OR/NOT gates, a rule should be made for every input fanning into a particular gate to delete the gate's output species with the opposite truth value to the input. If the output species has a unique $i \rightarrow j$ indexing, then only the input with the $i$th index can delete that output species.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c | c |}\hline
\textbf{AND Gate} & \textbf{OR Gate} & \textbf{NOT Gate} \\ \hline

$x_i^T + y_{i \rightarrow j}^F \rightarrow \emptyset$ & $x_i^T + y_j^F \rightarrow \emptyset$ & $x_i^T + y_j^T \rightarrow \emptyset$ \\ \hline
 
$x_i^F + y_j^T \rightarrow \emptyset$ & $x_i^F + y_{i \rightarrow j}^T \rightarrow \emptyset$ & $x_i^F + y_j^F \rightarrow \emptyset$ \\ \hline


\end{tabular}

\caption{\textit{(2, 0) rules for AND, OR, and NOT gates.}}\label{tab:(2,0)_AND_OR_NOT}
\end{center}
\end{table}

\subsubsection{Majority Gate}\label{2_0_majority_gates}

Let's consider the majority function when it has two unique input species, $T$ and $F$, where the counts of each species represent the amounts of true and false inputs, respectively. If $(|T| + |F|) \% 2 = 0$, then we should add an extra $F$ species before computing.

To compute the majority function with (2, 0) rules, we add a rule where the T and F species delete each other: $T + F \rightarrow \emptyset$. With this rule, all of the minority species will be deleted and some amount of the majority species will remain.

For implementing the majority gate in a circuit, given the inputs $x_i^b$ and output $y_i^b$, we must first convert the different input species into a new input species that share the same index before computing the majority function. If the amount of inputs fanning into a majority gate is even, then an extra false input should be fanned into that gate.

%To implement the majority gate in a circuit, we need to separate the input and output species. Instead of just the input species, $T$ and $F$, we also take the intermediate species $T_{i}$ and $F_{i}$. We also change our rules from $T + F \rightarrow \emptyset$ to $T_{i} + F \rightarrow \emptyset$ and $T + F_{i} \rightarrow \emptyset$.

%Before computing, if $(|T| + |F|) \% 2 = 0$, then we should add an extra $F_{i}$. To trigger the gate reaction we add in copies of each output species equal to half the input species, rounding down. After the rules are applied to this configuration, there will be either be only $F$ and $F_{i}$ or $T$ and $T_{i}$ To simplify the many $T_{i}$'s or $F_{i}$'s, we take a step.

%In the second step, we add one $T_{o}$ and one $F_{o}$ and execute the rules $T_{i} + F_{o} \rightarrow \emptyset$ and $F_{i} + T_{o} \rightarrow \emptyset$. This leaves us with either $T_{o}$ or $F_{0}$ representing our output.

To implement a majority gate in a circuit with (2, 0) rules, we must first convert all input species ($x_n^b$) fanning into the gate at index $i$ into a new species that share the same index, which we will call $a_i^b$. This will make it easier to compute the majority gate.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c  c | c | c |}\hline

\multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline

\textbf{1} & \textit{Add} & \makecell{$|f_i^{in}| \cdot a_i^T$ \\ $|f_i^{in}| \cdot a_i^F$} 

& \makecell{\vspace{-10pt} \\ $\forall j \in f_i^{in}:$ \\ $x_j^T + a_i^F \rightarrow \emptyset$ \\ $x_j^F + a_i^T \rightarrow \emptyset$ \\ \vspace{-9pt}}

& \makecell{$\forall j \in f_i^{in}$, convert $x_{j}^b$ input \\ species into $a_i^b$ species.} \\ \hline

%%%
\textbf{2} & \textit{Add} & \makecell{$\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^T$ \\ $\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^F$} 

& \makecell{$a_i^T + b_i^F \rightarrow \emptyset$ \\ $a_i^F + b_i^T \rightarrow \emptyset$}

& \makecell{Adding $\lfloor |f_i^{in}|/2 \rfloor$ amounts of $b_i^T$ and \\ $b_i^F$ species will delete all of the \\ minority species, leaving some amount \\ of the majority species remaining.} \\ \hline

%%%
\textbf{3} & \textit{Add} & \makecell{\vspace{-8pt} \\ $y_i^T$ \\ $y_i^F$ \\ \vspace{-10pt}} 

& \makecell{$a_i^T + y_i^F \rightarrow \emptyset$ \\ $a_i^F + y_i^T \rightarrow \emptyset$}

& \makecell{Convert $a_i^b$ into the proper output \\ species ($y_i^b$).} \\ \hline

\end{tabular}

\caption{\textit{(2, 0) rules for majority gates.}}\label{tab:(2,0)_MAJ}
\end{center}
\end{table}



\subsection{Examples}\label{3_0_examples}

\begin{figure}[!htbp]
    \centering
    {\includegraphics[width=5cm]{images/2depthformula.pdf}
    
    \caption{Example Formula.}\label{fig:(2,0)_example}
    }
\end{figure}

\input{2_0_example}



\subsection{Computing Formulas (Multiple-Input Model)}\label{2_0_computation}

\begin{theorem}\label{(2,0)_formula}
Boolean formulas (TC) can be computed with multiple input relaxed by a step CRN with only $(2,0)$ rules, O(G) species, O(D) steps, and O(G) volume.
    \end{theorem}
\begin{proof}
%\textit 
%Formulas are circuits in combination with only 2 inputs and 1 output. 2,0 does this in O(D), specifically steps=D+1. Each gate has unique input and output species. each step represents 1 level being solved. The gates reactions are triggered by the output species added at each step. The first level runs with the gate rules discussed in the gate section with one edit. In the case of an AND gate, there is not 2 z0's. there is 1 z0, and 1 z0*. z0 reacts with x1 inputs, and z0* interacts with y1 inputs. This removes the possibility of a gate producing 2z0 and the next gate running the reaction z0+output1 twice. Then we add the output species for the second layer and that layer's rules run, then the next step triggers, repeat. At the final layer, after the gate is solved, we need to narrow our solution to one answer. This is done by adding running an inverted not gate, Z0+true, Z0'+true and Z1+false,Z1'+false. This leaves only true or false, a single species output.

Section \ref{2_0_gates} explains how to compute TC gates. In order to run the formula, we need to convert the outputs into the inputs for the next gate. This can be done in a step by adding $x_i^T$ and $x_i^F$ for each gate at a given depth level and applying the reactions below.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c  c | c | c |}\hline

\multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline

\textbf{1} & \textit{Add} & \makecell{$x_i^T$ \\ $x_i^F$ \\} 

& \makecell{\vspace{-8pt} \\ $y_i^T + x_i^F \rightarrow \emptyset$ \\ $y_i^F + x_i^T \rightarrow \emptyset$ \\ $y_{j \rightarrow i}^T + x_i^F \rightarrow \emptyset$ \\ $y_{j \rightarrow i}^F + x_i^T \rightarrow \emptyset$ \\ \vspace{-8pt}}

& \makecell{Add species representing true and false \\ inputs and delete the species that are the \\ complement of the output. Now, only \\ the correct input species remains.} \\ \hline

\end{tabular}

\caption{\textit{(2, 0) rules for converting outputs to inputs per formula level.}}\label{tab:(2,0)_convert}
\end{center}
\end{table}

\textbf{Big-Oh Complexity Analysis:}
Having unique species to represent each gate in a Boolean formula results in O($G$) species.

All gates at a given depth level can be computed at the same time with a constant amount of steps, so a simulation of a Boolean formula would require O($D$) steps.

It is possible that not all species that are no longer needed will get deleted after computing a gate. For example, an AND gate with 3 false inputs would result in 3 $y_i^F$ and 2 false input species in the system. While this will not cause errors, it will increase the volume. Therefore, it is possible for only a fraction of the O($G$) species added throughout the simulation to be deleted, resulting in O($G$) volume.
\end{proof}

==> 2_0/main_leftovers.tex <==
\section{2,0 gates}

We now examine step CRNs with a ruleset consisting of (2, 0) rules. Decreasing the reactant count of the void rules causes some notable changes to the system's computation.

Section \ref{2_0_gates} shows how the computation of logic gates is still possible in stepped CRNs with (2, 0) rules. We then demonstrate with Theorem \ref{(2,0)_formula} how the system can compute TC \textit{formulas} (but not circuits) with $O$($G$) species, $O(D)$ steps, and $O(G)$ volume.

\subsection{Computing Logic Gates}\label{2_0_gates}
%(2, 0) CRNs are not capable of hard coding a two-input gate. We can not consider both inputs and destroy an output based on them. This limits us to reactions that only can include one of the inputs. Our solution is achieved by manipulating the outputs. given an and gate, any 1 input deletes a 0 output, and any 0 input deletes a 1 output. The number of 0 outputs is equal to the number of inputs because all inputs must be 1 for an and gate to not return 0.

The inputs of a binary gate that are constructed  in a step CRN system are  the same as in Section \ref{3_0_gates}. Let $f_i^{in}$ be the set of all the indexes of the inputs fanning into a gate at index $i$. Let $f_i^{out}$ be the set of all the indexes of the inputs fanning out of a gate at index $i$.

The outputs of gates in a step CRN system with (2, 0) rules are represented by either the species $y_n^b$ or $y_{i \rightarrow j}^F$.

\subsubsection{Basic Gates}\label{2_0_basic_gates}

Computing gates with (2, 0) rules requires a unique species to represent the inputs and outputs of each gate in a circuit. The species that have been used for computing a particular gate should never be used to compute a different gate. Figure \ref{fig:(3,0)_figure} \textit{(b)} shows a pattern the gates can be indexed in. For computing an AND gate, we add a single copy of the species representing a true output ($y_{j}^T$) and a species representing the false output for each input fanning in ($y_{i \rightarrow j}^F$, where $i$ is the index of the input). To compute an OR gate, we would add a species representing the true output for each input fanning in ($y_{i \rightarrow j}^T$) species and a single $y_{j}^F$ species. To compute NOT gates, we would just add one copy of each output species. For all AND/OR/NOT gates, a rule should be made for every input fanning into a particular gate to delete the gate's output species with the opposite truth value to the input. If the output species has a unique $i \rightarrow j$ indexing, then only the input with the $i$th index can delete that output species.

\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c | c |}\hline
\textbf{AND Gate} & \textbf{OR Gate} & \textbf{NOT Gate} \\ \hline

$x_i^T + y_{i \rightarrow j}^F \rightarrow \emptyset$ & $x_i^T + y_j^F \rightarrow \emptyset$ & $x_i^T + y_j^T \rightarrow \emptyset$ \\ \hline
 
$x_i^F + y_j^T \rightarrow \emptyset$ & $x_i^F + y_{i \rightarrow j}^T \rightarrow \emptyset$ & $x_i^F + y_j^F \rightarrow \emptyset$ \\ \hline


\end{tabular}

\caption{\textit{(2, 0) rules for AND, OR, and NOT gates.}}\label{tab:(2,0)_AND_OR_NOT}
\end{center}
\end{table}

\subsubsection{Majority Gate}\label{2_0_majority_gates}

Let's consider the majorit function when it has two unique input species, $T$ and $F$, where the counts of each species represent the amounts of true and false inputs, respectively. If $(|T| + |F|) \% 2 = 0$, then we should add an extra $F$ species before computing.

To compute the majority function with (2, 0) rules, we add a rule where the T and F species delete each other: $T + F \rightarrow \emptyset$. With this rule, all of the minority species will get  deleted and some amount of the majority species will remain.

To implement the majority gate in a circuit, given the inputs $x_i^b$ and output $y_i^b$, we must first convert the different input species into a new input species that share the same index before computing the majority function. If the amount of inputs fanning into a majority gate is even, then an extra false input should be fanned into that gate.

To implement the majority gate in a circuit, we need to separate the input and output species. Instead of just the input species, $T$ and $F$, we also take the intermediate species $T_{i}$ and $F_{i}$. We also change our rules from $T + F \rightarrow \emptyset$ to $T_{i} + F \rightarrow \emptyset$ and $T + F_{i} \rightarrow \emptyset$.

Before computing, if $(|T| + |F|) \% 2 = 0$, then we should add an extra $F_{i}$. To trigger the gate reaction we add in copies of each output species equal to half the input species, rounding down. After the rules are applied to this configuration, there will be either be only $F$ and $F_{i}$ or $T$ and $T_{i}$ To simplify the many $T_{i}$'s or $F_{i}$'s, we take a step.

In the second step, we add one $T_{o}$ and one $F_{o}$ and execute the rules $T_{i} + F_{o} \rightarrow \emptyset$ and $F_{i} + T_{o} \rightarrow \emptyset$. This leaves us with either $T_{o}$ or $F_{0}$ representing our output.

To implement a majority gate in a circuit with (2, 0) rules, we must first convert all input species ($x_n^b$) fanning into the gate at index $i$ into a new species that share the same index, which we will call $a_i^b$. This will make it easier to compute the majority gate.

%(I don't know how this table works)
\begin{table}[H]
\begin{center}
\begin{tabular}{| c | c  c | c | c |}\hline

\multicolumn{3}{|c|}{\textbf{Steps}} & \textbf{Relevant Rules} & \textbf{Description} \\ \hline

\textbf{1} & \textit{Add} & \makecell{$|f_i^{in}| \cdot a_i^T$ \\ $|f_i^{in}| \cdot a_i^F$} 

& \makecell{\vspace{-10pt} \\ $\forall j \in f_i^{in}:$ \\ $x_j^T + a_i^F \rightarrow \emptyset$ \\ $x_j^F + a_i^T \rightarrow \emptyset$ \\ \vspace{-9pt}}

& \makecell{$\forall j \in f_i^{in}$, convert $x_{j}^b$ input \\ species into $a_i^b$ species.} \\ \hline

%%%
\textbf{2} & \textit{Add} & \makecell{$\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^T$ \\ $\lfloor |f_i^{in}|/2 \rfloor \cdot b_i^F$} 

& \makecell{$a_i^T + b_i^F \rightarrow \emptyset$ \\ $a_i^F + b_i^T \rightarrow \emptyset$}

& \makecell{Adding $\lfloor |f_i^{in}|/2 \rfloor$ amounts of $b_i^T$ and \\ $b_i^F$ species will delete all of the \\ minority species, leaving some amount \\ of the majority species remaining.} \\ \hline

%%%
\textbf{3} & \textit{Add} & \makecell{\vspace{-8pt} \\ $y_i^T$ \\ $y_i^F$ \\ \vspace{-10pt}} 

& \makecell{$a_i^T + y_i^F \rightarrow \emptyset$ \\ $a_i^F + y_i^T \rightarrow \emptyset$}

& \makecell{Convert $a_i^b$ into the proper output \\ species ($y_i^b$).} \\ \hline

\end{tabular}

\caption{\textit{(2, 0) rules for majority gates.}}\label{tab:(2,0)_MAJ}
\end{center}
\end{table}



\textbf{Big-Oh Complexity Analysis:}
Having unique species to represent each gate in a Boolean formula results in O($G$) species.

All gates at a given depth level can be computed at the same time with a constant amount of steps, so a simulation of a Boolean formula would require O($D$) steps.

It is possible that not all species that are no longer needed will get deleted after computing a gate. For example, an AND gate with 3 false inputs would result in 3 $y_i^F$ and 2 false input species in the system. While this will not cause errors, would increase the volume. Therefore, it is possible for only a fraction of the O($G$) species added throughout the simulation to be deleted, resulting in O($G$) volume.
\end{proof}


%\end{document}


\begin{theorem}\label{(2,0)_circuit}
Boolean circuits (AMNO) can be computed with multiple input relaxed by a step CRN with only (2, 0) rules, O(G) species, O(D) steps, and O(${F_{out}}^D$) volume.
\end{theorem}
\begin{proof}
\textit 
To handle circuits, a CRN must handle fan out. The simplest way to handle fan out is to copy it and everything underneath it into 2 sections. One is to simulate one output of the gate, and another is  to simulate the other output of the gate. All this truly does is drag the fan out back to the beginning, but if given enough copies of the inputs, this can be done. It comes at the cost of 2 to the depth power species because each new set of identical gates must have different species. It is more efficient to not divide the circuit, but instead run more inputs through each gate. A 2,0 step crn cannot double something, but it can, given twice the inpts, create twice as much of it.If we put 4 inputs into an and gate by using there rules (need picture of professor bins 2,0 solution below this) instead of two, we end up with 2 outputs. by adding a step to separate the two, we can reset the next level to simply have normal inputs. This simulates circuits in volume = 2 to depth instead of species = 2 to depth because we do not need new species for each fanout, only more of the inputs. The specific metrics are 4Depth steps, 6Gate species, and 2 to the depth power volume. This method is unnatural because it requires more then 1 copy of each input bit.

There is no known way to duplicate a single species with only (2, 0) rules and strict computing. So, to create enough copies of the output of a gate that fans out, we must increase the count of the inputs to match the count of the gate or sum of gates it is being inputted into. For instance, if a gate needs $k$ copies of its output species to fan out, each of the gates that are inputs for that gate also needs $k$ copies of their output species, and each of the gates that are inputs for those gates needs $k$ copies, and so on. The counts of the species that are added in each step ($x_i^b$ and $y_i^b$) also need to be multiplied by the number of output species a given gate needs.

\textbf{Big-Oh Complexity Analysis:} The species and steps Big-Oh complexity (O(G) and O(D), respectively) remain unchanged from the method used to compute formulas because no new species or steps are being introduced.

The volume of the system could grow exponentially based on the depth and the size of the max fan out. For instance, if the primary inputs were inputted into a gate that had a fan out of $k$, and that gate fanned out into other gates that had a fan out of $k$, and this pattern continued for most of the circuit, then the primary input species' count would need to be multiplied by $k$ for the amount of depth levels this pattern continued. Therefore, where $F_{out}$ is the max fan out of a circuit, then a circuit simulation could require a O(${F_{out}}^D$) volume.
\end{proof}

\section{Lower Bound}


\newcommand{\stablelysimulated}{{stablely simulate}}

\begin{definition}\label{natural-simulation-def}
A circuit is {\it \stablelysimulated d} by a step CRN if each gate $g$ is assigned $c_{1,g}$ copies of species $1_g$ to represent $1$ as output each,  and $c_{0, g}$ copies of $0_g$ to represent $0$ output each. When gate $g$ gives an output, it will be either $c_{1,g}$ copies of species $1_g$ for the case $1$, or $c_{0,g}$ copies of species $0_g$ for the case $0$. We define  $C(g)=c_{1,g}+c_{0,g}$ to count the number of copies used for gate $g$.
There is a special case that $g$ is one of the input bits. 

If a circuit $C(.)$ compute a function $f(x_1\cdots x_n)=y_1\cdots y_m$ and $C(.)$ is \stablelysimulated~by a step CRN, define $1_{f(.),i}$ to represent the case $y_i$ to be $1$ and $0_{f(.),i}$ to represent the case $y_i$ to be $0$.
  \end{definition}

  By Definition~\ref{natural-simulation-def}, when gate $g$ outputs $1$, it has $c_{1,g}$ copies of $1_{g}$ to enter the next layer, and all the $c_{0,g}$ copies of $0_g$ are removed. 



%\subsection{Volume Lower Bounds }

In this section, we derive an exponential lower bound for the volume in a step CRN with $(2,0)$ rules  to simulate boolean circuits of depth $D$. Our lower bound almost matches the upper bound. 

The idea to prove the lower bound is to design a circuit that will be simulated by any step CRN with only $(2,0)$ rules. It has $D$ stages such that each stage of the circuit has $O(1)$ layers. We establish a recursive inequality among the volume for three consecutive stages. It implies an exponential lower bound for some species in the input stage.

\begin{lemma}\label{basic-lemma}
Assume that  a step CRN with $(2,0)$ rules simulates a circuit $C(.)$. Let $b\in \{1_g, 0_g\}$ be an output species.  Then if one copy of a species is removed or added, it brings at most one difference for the number of copies for the species $b$. 
\end{lemma}
\begin{proof}
  We prove it via induction over the total start volume. If the volume is zero or one in the beginning, it is trivial. Assume it is true when the start volume is at most $n$. Consider the start volume to be $n+1$. Let species $u$ lose one copy. Let $u+v\rightarrow \emptyset$ be applied (otherwise, it is trivial). We transform the problem into adding one copy of $v$ into a step CRN with volume $n-1$. This case is proved by inductive hypothesis. The case by adding one copy of $u$ is similar.
\end{proof}

\begin{lemma}\label{fundamental-lemma}
Let $f(x_1,\cdots, x_n)=y_1\cdots y_m$ be a function such that each variable $x_i$ or $y_j$ has value in $\{0,1\}$. If a step CRN with $(2,0)$-rules to compute $f(.)$, and flipping variable $x_j$ will flip the values at $y_{i_1},\cdots, y_{i_t}$, then $C(x_j)\ge \sum_{k=1}^t C(y_{i_k})$. %where $C(u)$ represents the number of copies of a species to represent variable $u$.
\end{lemma}

\begin{proof}
Assume that there is a step CRN to simulate $f(.)$.
 Assume $C(x_j)< \sum_{k=1}^t C(y_{i_k})$.
For each boolean variable $x$, we also use $x$ to represent the gate that outputs the value of $x$.

When one copy is removed in the input side, it may add or decrease at most one copy on the output side by Lemma~\ref{basic-lemma}.
When one copy is added in the input side, it may add or decrease at most one copy on the output side  by Lemma~\ref{basic-lemma}. 

If the output side need to change it value from $a\in \{0,1\}$ to $1-a$, it needs to remove all the copies that represent the current $a$ and add the new copies that represent the value $1-a$.
Assume that the current $x_j$ has value $a\in\{0,1\}$. Consider the transitions of two phases:



Phase 1: Remove $c_{a, x_j}$ copies $x_j$.

After $x_j$ is removed, it affects at most $c_{a, x_j}$ copies of species $y_{i_1},\cdots, y_{y_t}$ by Lemma~\ref{basic-lemma}.


Phase 2: Add $c_{1-a, x_j}$  copies $x_j$ with  value $1-a$ over input side. 

After adding $c_{1-a, x_j}$ copies of $x_j$ (with flipped value), it affects at most $c_{1-a, x_j}$ copies of species $y_{i_1},\cdots, y_{y_t}$ by Lemma~\ref{basic-lemma}.

The output side needs to destroy the old copies for the species for $y_{i_1},\cdots, y_{i_t}$, and add new copies for $y_{i_1},\cdots, y_{i_t}$. But the two phases can only affect at most $C(X_j)=c_{a, x_j}+c_{1-a, x_j}< \sum_{k=1}^t C(y_{i_k})$ copies in the output side. 
 This brings a contradiction.

\end{proof}

\begin{definition}
A list of boolean circuits $\{H_n(.)\}$ is uniform if there is a Turing machine $M(.)$ such that each $H_n(.)$ can be generated by $M(1^n)$ in a polynomial $p(n)$ steps.    
\end{definition}

\begin{theorem}\label{(2,0)-lower-thm} There is a uniform boolean circuits $\{V_D(x_1, x_2, x_3)\}_{D=1}^{+\infty}$ such that each $V_D(x_1, x_2, x_3)$ has depth $O(D)$, size $O(D)$ and three output bits, and 
   it requries $C(g)=2^{\Omega(D)}$ for at least one input gate $g$ in a step CRN with $(2,0)$ rules to \stablelysimulated~$V_D(.)$. 
   %For all $D > 0$, there e
\end{theorem}

\begin{proof}
%It can be proved via an induction of the %depth $D$. It is trivial when $D=1$. %Assume that it needs $2^{c(D-1)}$ volume %on the input side to simulate a circuit %of depth $D-1$, where $c\in (0,1)$ is %fixed. 
We construct a circuit that has $O(D)$ layers. It is built in $D$ stages. Each stage has a circuit of depth $O(1)$ to compute function $s(x_1, x_2, x_3)=y_1y_2y_3$.

The function $s(.)$ has the properties: 
\begin{eqnarray}
s(1,1,1)&=&111,\\
s(0,1,1)&=&000,\label{x1-y4-ineqn} \\
s(1,0,1)&=&011,\label{x2-y1-ineqn}\\
s(1,1,0)&=&101,\label{x3-y2-ineqn}\\
s(0,0,0)&=&110.
\end{eqnarray}

%The output of the circuit is the four output bits of the final layer. For the input $(1,1,1)$, the first bit $x_1$ goes $1\rightarrow 0$, it affect $y_4$ to go $1\rightarrow 0$. Therefore, it lets the output go from $111$ to $000$. The last layer $D$ has at least three bits in output. Thus, it requires at least $3$ copies for $y_4$. Thus, it needs at least $3$ copies of $x_1$ since it affects $y_4$.

%Let the boolean function $s(x_1, x_2, x_3)=x_1'x_2'x_3'$, where $x_1', x_2'$ and %$x_3'$ are defined as above. 
Define function $s^{(1)}(x_1, x_2, x_3)=s(x_1, x_2, x_3)$ and $s^{(k+1)}(x_1, x_2, x_3)=s(s^{(k)}(x_1, x_2, x_3))$ for all integers $k>1$. The circuit $V(x_1, x_2, x_3)=s^{(D)}(x_1, x_2, x_3)$. We can also represent the circuit $V(x_1, x_2, x_3)=s^{(D)}(x_1, x_2, x_3)=s_{D-1}\circ s_{D-2}\circ\cdots s_0(x_1, x_2, x_3)$, where $s_i(.)$ represent the function $s(.)$ at stage $i$. The circuit $V(x_1, x_2, x_3)$, which computes $s^{(D)}(x_1,x_2, x_3)$, is to link the $D$ circuits $V_s(x_1, x_2, x_3)$ that computes function $s(x_1, x_2, x_3)$.
The three output bits for $s_k(.)$ at stage $k$ becomes three input bits of $s_{k-1}(.)$ at stage $k-1$.

Let the output of the circuit  be stage $0$. The input stage has the largest stage index.
Consider the general case. Let $C_k(u)$ be the number of copies of variable $u$ in stage $k$. Let $v_{i, k}$ be the variable $v_i$ at stage $k$. Clearly, $C_D(y_{1,0})\ge 1, C_D(y_{2,0})\ge 1, C_D(y_{3,0})\ge 1$. We have $C_k(x_{1,k})\ge  C_k(y_{1,k})+C_k(y_{2,k})+C_k(y_{3,k})$ by equation (\ref{x1-y4-ineqn}), $C_k(x_{2,k})\ge C_k(y_{1,k})$ by equation (\ref{x2-y1-ineqn}), and $C_k(x_{3,k})\ge C_k(y_{2,k})$ by equation (\ref{x3-y2-ineqn}). Note that $y_{i, k}$ is equal to $x_{i, k-1}$ as the output of the $S_{k}(.)$ becomes the input of $s_{k-1}(.)$
We also have $C_k(y_{i, k})\ge C_{k-1}(x_{i, k-1})$ for $i=1,2,3$, and $C_k(y_{4, k})\ge C_{k-1}(x_{1, k-1})+C_{k-1}(x_{2, k-1})+C_{k-1}(x_{3, k-1})$ by Lemma~\ref{fundamental-lemma}.
We also have $C_k(y_{i, k})\ge C_{k-1}(x_{i, k-1})$ for $i=1,2,3$  by Lemma~\ref{fundamental-lemma}.
In each stage, the input to the function $s(.)$ can reach all the cases $000,011,101,110,111$
by adjusting the three bits of the input of the circuit. In particular, when the input is $111$, the function $s(,)$
gives the same output $111$
at all phases.

%Apply Lemma~\ref{fundamental-lemma} and inductive hypothesis. 
A simple repetition of the above inequalities, we derive a $2^{\Omega(D)}$ volume lower bound.

\begin{eqnarray}
 C_k(x_{1, k})  &\ge& C_{k-1}(x_{1, k-1})+C_{k-1}(x_{2, k-1})+C_{k-1}(x_{3, k-1})\\
 &\ge& C_{k-1}(x_{1, k-1})+C_{k-1}(y_{1, k-1})\\
  &\ge& C_{k-1}(x_{1, k-1})+C_{k-2}(x_{1, k-2}).
\end{eqnarray}
Let $a_0, a_1,\cdots$ be the Fibonacci series with $a_0=a_1=1$ and recursion $a_{k}=a_{k-1}+a_{k-2}$ for all $k>1$. Clearly, we have $C_{k}(x_{1,k})\ge a_k$ for all $k\ge 0$.  %It is well known that the items in a Fibonacci series have exponential lower bound.
The theorem is proved.


{\bf More details in the proof will be added by Bin Fu.    }
\end{proof}

==> 2_0_formula_example.tex <==
% Here we go!
\begin{table}[t]
%\vspace{-.1cm}
\renewcommand{\arraystretch}{.5}
\begin{center}
\begin{tabular}{| c | c  c | c |}\hline
    \multicolumn{4}{|c|}{\textbf{Initial Configuration: $y_1^T$, $y_2^F$, $y_3^F$, $y_4^T$}} \\ \hline

    \multicolumn{3}{|c|}{\textbf{Step}} & \textbf{Relevant Rules} \\ \hline
    
    \textbf{1} & \textit{Add} & \makecell{$x_1^T$, $x_2^T$, $x_3^T$, $x_4^T$ \\ $x_1^F$, $x_2^F$, $x_3^F$, $x_4^F$} 
    
    & \makecell{\vspace{-10pt} \\ $y_1^T + x_1^F \rightarrow \emptyset$ \\ $y_2^F + x_2^T \rightarrow \emptyset$ \\ $y_3^F + x_3^T \rightarrow \emptyset$ \\ $y_4^T + x_4^F \rightarrow \emptyset$ \\ \vspace{-9pt}} \\ \hline
    
    %%%
    \textbf{2} & \textit{Add} & \makecell{$y_5^T$, $y_{1 \rightarrow 5}^F$, $y_{2 \rightarrow 5}^F$ \\ $y_6^T$, $y_{3 \rightarrow 6}^F$, $y_{4 \rightarrow 6}^F$} 
    
    & \makecell{$x_1^T + y_{1 \rightarrow 5}^F \rightarrow \emptyset$ \\ $x_2^F + y_5^T \rightarrow \emptyset$ \\ $x_3^F + y_6^T \rightarrow \emptyset$ \\ $x_4^T + y_{4 \rightarrow 6}^F \rightarrow \emptyset$} \\ \hline
    
    %%%
    \textbf{3} & \textit{Add} & \makecell{$x_5^T$, $x_6^T$ \\ $x_5^F$, $x_6^F$} 
    
    & \makecell{\vspace{-10pt} \\ $y_{2 \rightarrow 5}^F + x_5^T \rightarrow \emptyset$ \\ $y_{3 \rightarrow 6}^F + x_6^T \rightarrow \emptyset$ \\ \vspace{-9pt}} \\ \hline

    %%%
    \textbf{4} & \textit{Add} & \makecell{$y_{5 \rightarrow 7}^T$, $y_{6 \rightarrow 7}^T$, $y_7^F$} 
    
    & \makecell{\vspace{-10pt} \\ $y_{5 \rightarrow 7}^F + x_5^T \rightarrow \emptyset$ \\ $y_{6 \rightarrow 7}^F + x_6^T \rightarrow \emptyset$ \\ \vspace{-9pt}} \\ \hline

    %%%
    \textbf{5} & \textit{Add} & \makecell{\vspace{-8pt} \\ $x_7^T$, $x_7^F$ \\ \vspace{-10pt}} 
    
    & \makecell{$y_7^F + x_7^T \rightarrow \emptyset$} \\ \hline
    
\end{tabular}

\caption{\textit{(2, 0) rules and steps for computing the formula in Figure \ref{fig:(2,0)_example}.}
%\vspace{-.7cm}
}\label{tab:(2,0)_formula_example}
\end{center}
%\vspace{-.8cm}
\end{table}

We now demonstrate a simple example of computing a threshold formula. The formula has four inputs: $x_1$, $x_2$, $x_3$, and $x_4$. At the first depth level, $x_1$ and $x_2$ fan into an AND gate, and likewise for $x_3$ and $x_4$. Both outputs are then fanned into an OR gate, whose output represents the final value of the formula. 

The initial configuration consists of the input species. Step 1 converts the inputs into input species. Step 2 then performs all gate operations at the first depth level. Step 3 converts the output species into input species for the next depth level. Step 4 computes the final gate. Finally, Step 5 coverts the output into an input species that represents the final output of the formula. A more detailed explanation of computing the formula is in Table.

==> TODO.tex <==
To-do list
These are things that currently need to be done for this paper before the final version (4/24).
Check off something when you fix it and add your initials + a brief description of how you fixed it.
-Rachel

TO-DO
---------------------------------------------------------------------------------

Review 1 
---------------------------
[X] Make full example: "The main issue I have with the paper is presentation. I have a very difficult time understanding the construction, because the examples are not worked out fully. I think a single full example step CRN computing the formula in Fig. 1 would do more to communicate how it works than all of Section 3."

(We could look into doing an formula example section like in the MCU paper. The 15-page limit could be an issue, however. - A.M.)

Note: Schweller suggested the possibility of removing some technical proofs in favor of visual examples for the conference. - A.M.

Added a subsection detailing an example computation of a formula. - A.M.

[x] Edit intro: "page 1: Chemical Reaction Networks (CRNs) are a well-established model of self-assembly.
That doesn't sound right. It's true that self-assembly systems such as the kinetic Tile Assembly Model can be described as a type of CRN, but that's just one use of the CRN model. They can also describe systems in which the species are not simply bigger and bigger polymers that can assemble. I would just say they are a well-established model of chemistry."

Changed "self-assembly" to "chemistry". -RA

[X] add def to intro: "I would state in the introduction what you mean by "volume". I'd also given a simple example of a step CRN (e.g., an informal definition by example), so the introduction is more self-contained."

I have imported the step CRN example image and added it commented out in the preliminaries above 2.3. If we have space for this, feel free to uncomment it -RA
(We could add the step CRN figure from the MCU paper - A.M.)
I added it in. For now, let's try and add all of what the reviewers suggested without worry for space. Afterwards, we can check what could be axed OR let Wylie do his magic. - A.M.
May still need to define volume

[x] Update description: "I would suggest using the term "reaction" rather than "rule", since every other paper on the model of chemical reaction networks calls these "reactions"."

Added to intro in bimolecular void rules section: "In this paper, we use the terms \emph{reaction} and \emph{rule} interchangeably to denote a reaction rule." -RA

[X] Add definition: "Table 1 should define G, D, and GFoutD."

Added definitions for circuit properties in the table. - A.M.

[x] Update figure: "I find Figure 1 strange. There's a picture of a circuit, but no explanation of how it is being simulated by a CRN. I think it would make more sense to just show part (a) at this point unless you're going to say something else about the relationship of the circuit to the CRN (e.g., that you will have "wire" species for wires 5, 6, 7, or something)."

Updated Figure 1b with input bit truth values to specifically use the ones we show in Figure 1a. Updated the captions of these figures to reflect this. I am unsure if I should also add the truth value of the output bit, for simplicity I didn't for the time being. -RA

[X] Update figure: "I think in figures like 2, the black lines represent reactions, i.e., this one has reactions $y_3^T$ + $x_2^F$ --> nothing and $y_{1-->3}^F$ + $x_1^T$ --> nothing, but that's not entirely clear from the phrase "represents their removal from the system."

Altered caption to say "The black lines connecting species represents a reaction applied to them." - A.M.
 
[X] Update figure and description: "I also think Figure 2 should be more complete. For example, the paragraph down the page mentions species such as $y_i^T$ that do not appear in the figure. I think figures are best when they are as self-contained as possible, both in showing everything in the picture, and having a caption that tries to give as much information as possible (but main text can be used to avoid an excessively long caption). This construction is simple enough that the figure diagram and caption could completely explain the idea without the reader needing to go to the main text at all. In fact, I'd suggest to make it four parts: current part (a), part (b) is a full description of the reactions and molecules to add at each step, and part (c) is something like the current part (b), showing it in action on a particular input where the answer is false, and part (d) should be similar to part (c) but on the input (true, true), to show how it works when the answer should be true. You might also consider making this a 3-input AND gate; I get the feeling that the generalization to more inputs will be more obvious from that example than from the 2-input example."

In progress - A.M.
Added updated and additional figures for fig 2 (now 3) and updated caption. The formatting is bad sorry please feel free to change it-RA

[X] Add detail to example: "You have a paragraph "AND gate example", which does partially describe a 3-input AND gate, but the example is not complete. You state what species are involved, but then just say "The rules described in Table 2 are then applied." What's the point of an example if you're going to just point the reader to the full construction and tell them to read that? If this example is to be helpful, you have to give the explicit list of reactions. I think in this case it would be
x_1^T + y_{1->1}^F -> nothing
x_2^T + y_{2->1}^F -> nothing
x_3^T + y_{3->1}^F -> nothing
x_1^F + y_{1}^T -> nothing
x_2^F + y_{1}^T -> nothing
x_3^F + y_{1}^T -> nothing
I'm also quite confused because if the three inputs have indices 1, 2, 3, then why does the output also have index 1?"

Updated output species to have the correct output index of 4 instead of 3. Also listed the rules being applied to the system. - A.M.

[X] Clarify indexing and wires: "In particular, you name input species for a gate with x, but outputs for the gate with y. But the outputs need to interact with downstream gates. Where are the reactions for the y outputs to influence the next gate to which that wire is an input?
I find this construction quite difficult to understand without a complete, worked out example. I'm also realizing I'm confused how these are wired together. I suggest writing out the full set of reactions for Fig. 1 (you can simplify it to have two gates, but it needs to have at least 2)."

Is he talking about depth traversal? - A.M.

Updated indexing definition with better clarification.

[x] Summarize table: "Table 2 is then your formal description of the full way to do all these logic gates, but having an example "legend" of a revised Figure 2 will make it more easy to see how it's working."
Revised figure 2 and caption as above -RA

[ ] Update bib: "Some bibliography refs like [1,2] do not state the venue. I'm assming it's arXiv? If so state that and give the arXiv ID."

Citations that may need more info: [5], [21], [24]

Review 2
----------------------------------
[x] Fix formatting: "p.5, l.15: 0 and 1 are used as superscripts here, but T and F are used later in Section 3.1."

(Referring to the input-strict computing definition) Changed the 0 and 1 superscripts to F and T, and did the same in the multiple input relaxation definition following it. Left original versions commented out just in case and to verify I changed them correctly. I think all the superscripts are consistent now? -RA

[~] Fix grammar, possibly clarify: "p.7, l.-2: The same index 1 is used in different places."

This might be referring to the examples/figures? Those have been fixed. - A.M.

[ X] Clarify claim: "p.12, Lemma 2: It is unclear how the claim "there are at most t copies of a species affected that represent y_i" is treated in the proof by contradiction. It is also unclear how this claim is used later in Theorem 3."

Revisions were made for this comment by Bin Fu.



[ X] Look into: "p.13, (6): Should the leftmost occurrence of D be 0?"

Revisions were also made for this comment by Bin Fu.


Review 3
--------------------------------------
[-] Need to think about (could require more effort): "The most apparent drawback for this proposal is that fan-outs can only be implemented by duplicating the gates (adding more copies of the input and gate molecules). The number of duplicates required depends on all down-stream fan-outs and thus could be proportional to the size of the circuit even if all gates of constant fan-outs."

[-] Also need to think about: "Focusing on the two-reaction zero-product reactions essentially implies that there is no amplification. This results in the above fan-out problem and also may cause issues in the control of volume. Although it really seems easy to implement, it is unclear whether it is a good set of reactions to study."

Talking with Schweller about the above two issues, the former is essentially only an observation about our system construction (which we prove too) and the later is just implying the reviewer doesn't really care about our choice of reactions. To that end, I wouldn't place much thought into them. - A.M.

[X] Update defintion: "The current definition of step CRNs require that a terminal state being reached before the next step. However, only a small fraction of CRNs can guarantee the reachability of terminal states. I think the definition would be more valuable if it applies to more general classes of CRNs."

Proposal: Include to conclusions/future work a discussion about a relaxation to the step CRN model where moving to the next step does not require reaching a terminal state. - A.M.

Updated the conclusion to add relaxation to our step CRN model as a possible future direction. - A.M.

Other changes
--------------------------------------
[X] In abstract, changed "polynomial resources" to "linear resources." - A.M.
